Nonparametric test for a constant beta between \Ito semi-martingales based on high-frequency data

We derive a nonparametric test for constant beta over a fixed time interval from high-frequency observations of a bivariate \Ito semimartingale. Beta is defined as the ratio of the spot continuous covariation between an asset and a risk factor and the spot continuous variation of the latter. The test is based on the asymptotic behavior of the covariation between the risk factor and an estimate of the residual component of the asset, that is orthogonal (in martingale sense) to the risk factor, over blocks with asymptotically shrinking time span. Rate optimality of the test over smoothness classes is derived.

==> debris.tex <==
An alternative version of the test can be formulated as follows.
We set
\begin{equation}
S_j^n(\beta) = \frac{k_n(1+T_j^n(\beta))}{k_n-1-T_j^n(\beta)}.
\end{equation}
Then we can use the fact that the leading term of $S_j^{n}(\beta)$, i.e., the one under constant volatility over the block is the square of random variable with $t$-distribution and $k_n$ degrees of freedom. This leads to a better finite sample approximation of the statistic over the block.
\begin{cor}
Suppose assumption A holds and $k_n = o(n^{1/3})$. Then if $\beta_t = \beta_0$ for $t\in[0,1]$
\begin{equation}
\frac{k_n-2}{k_n}\sqrt{\frac{k_n-4}{2k_n-2}}\sqrt{\frac{n}{k_n}}\sum_{j=1}^{\lfloor \frac{n}{k_n}\rfloor}\left[S_j^n(\beta_0) - \frac{k_n}{k_n-2}\right]~\stackrel{\mathcal{L}-s}{\longrightarrow}~Z,
\end{equation}
where $Z$ is standard normal defined on an extension of the original probability space.
\end{cor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We use the following shorthand notation
\begin{equation}
\widetilde{Y}_t^c = \int_0^t(\alpha_s^Y-\beta^n\alpha_s^X)ds+\int_0^t\widetilde{\sigma}_sd\widetilde{W}_s,
\end{equation}
where for simplicity we have suppressed the dependence of $\widetilde{Y}_t^c$ on $n$. Upon denoting $\epsilon^n = \beta^n-\beta_0$, we can then simplify
\begin{equation}
\Delta_i^nY^c-\beta^n\Delta_i^nX^c = \Delta_i^n\widetilde{Y}^c+\epsilon^n\Delta_i^nX^c.
\end{equation}
\begin{lema}\label{lema_mean}
Under assumption SA and $\beta_t=\beta_0$ for $t\in[0,1]$, we have
\begin{equation}
\left| \mathbb{E}_{\frac{(j-1)k_n}{n}}\left( C_j^n(\beta^n)^2 - V_j^n(\beta^n) \right) \right|\leq K\left(\epsilon_n^2k_n+\frac{\epsilon_n}{k_n}+\frac{\epsilon_nk_n}{\sqrt{n}}+\frac{k_n}{n}+\frac{1}{\sqrt{n}}\right).
\end{equation}
\end{lema}
\textbf{Proof of Lemma~\ref{lema_mean}.}
First, we list some auxiliary bounds. By using $\langle W,\widetilde{W}\rangle_t = 0$ and the \Ito semimartingale assumption for $\alpha_t$, we have
\begin{equation}
|\mathbb{E}_{i-1}^n(\Delta_i^nX^c\Delta_i^n\widetilde{Y}^c)|\leq \frac{K}{n^2}.
\end{equation}
Using \Ito lemma for $(\Delta_j^nX^c)^2$, the \Ito semimartingale assumption for $\sigma_t$ and $\langle W,\widetilde{W}\rangle_t = 0$, we have
\begin{equation}
|\mathbb{E}_{i-1}^n(\Delta_i^nX^c\Delta_i^n\widetilde{Y}^c(\Delta_j^nX^c)^2)|\leq \frac{K}{n^2\sqrt{n}},~~\textrm{for $i<j$}.
\end{equation}
Using \Ito lemma
\begin{equation}
\mathbb{E}_{i-1}^n(\Delta_i^nX^c)^4\leq \frac{K}{n^2}.
\end{equation}
Using \Ito lemma for $(\Delta_j^nX^c)^3$, the \Ito semimartingale assumption for $\sigma_t$ and $\langle W,\widetilde{W}\rangle_t = 0$, we have
\begin{equation}
|\mathbb{E}_{i-1}^n(\Delta_i^nX^c)^3\Delta_i^n\widetilde{Y}^c)|\leq \frac{K}{n^2\sqrt{n}}.
\end{equation}
Using these bounds, and applying \Ito lemma, we easily get
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left(C_j^n(\beta^n)\right)^2 = \frac{n^2}{k_n}\sum_{i=(j-1)k_n+1}^{jk_n}\mathbb{E}_{\frac{(j-1)k_n}{n}}
\left(\int_{(i-1)\Delta_n}^{i\Delta_n}\sigma_s^2ds\int_{(i-1)\Delta_n}^{i\Delta_n}\widetilde{\sigma}_s^2ds\right)+\widetilde{R}_j^{(n,1)},
\end{equation}
where
\begin{equation}
|\mathbb{E}_{\frac{(j-1)k_n}{n}}(\widetilde{R}_j^{(n,1)})|\leq K\left(\epsilon_n^2k_n+\frac{\epsilon_nk_n}{\sqrt{n}}+\frac{k_n}{n}+\frac{1}{\sqrt{n}}\right).
\end{equation}
Using \Ito lemma, we can write
\begin{equation}
\begin{split}
V_j^n(\beta^n) &= \frac{n^2}{k_n^2}\left(2\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}X_s^ndX_s^c+ \int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_s^2ds \right)
\\&~~~\times
\left(2\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}(\widetilde{Y}_s^n+\epsilon_nX_s^n)d(\widetilde{Y}_s^c+\epsilon_nX_s^c)+ \int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}(\widetilde{\sigma}_s^2+\epsilon_n^2\sigma_s^2)ds \right),
\end{split}
\end{equation}
where we denote
\begin{equation}
X_s^n = X_s^c-X_{\frac{i-1}{n}}^c,~~~\widetilde{Y}_s^n = \widetilde{Y}_s^c-\widetilde{Y}_{\frac{i-1}{n}}^c,~~\textrm{for $i\in\left[\frac{i-1}{n},\frac{i}{n}\right]$}.
\end{equation}
Using the above decomposition, as well as the fact that $\sigma_t^2$ and $\widetilde{\sigma}_t^2$ are \Ito semimartingales, we get
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left(V_j^n(\beta^n)\right) = \frac{n^2}{k_n^2}\mathbb{E}_{\frac{(j-1)k_n}{n}}
\left(\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_s^2ds\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}(\widetilde{\sigma}_s^2+\epsilon_n^2\sigma_s^2)ds\right)
+\widetilde{R}_j^{(n,2)},
\end{equation}
where
\begin{equation}
|\mathbb{E}_{\frac{(j-1)k_n}{n}}(\widetilde{R}_j^{(n,2)})|\leq K\left(\frac{\epsilon_n}{k_n}+\frac{1}{\sqrt{n}}\right).
\end{equation}
Given the bounds for the conditional expectations of the residuals $\widetilde{R}_j^{(n,1)}$ and $\widetilde{R}_j^{(n,2)}$, we are left with the difference
\[\frac{n^2}{k_n}\sum_{i=(j-1)k_n+1}^{jk_n}\mathbb{E}_{\frac{(j-1)k_n}{n}}
\left(\int_{\frac{i-1}{n}}^{\frac{i}{n}}\sigma_s^2ds\int_{\frac{i-1}{n}}^{\frac{i}{n}}\widetilde{\sigma}_s^2ds\right) - \frac{n^2}{k_n^2}\mathbb{E}_{\frac{(j-1)k_n}{n}}
\left(\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_s^2ds\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\widetilde{\sigma}_s^2ds\right).\]
Using the \Ito semimartingale representation of $\sigma_t^2$ and $\widetilde{\sigma}_t^2$, as well as \Ito formula for the function $f(x,y)=xy$, we have
\begin{equation}
|\mathbb{E}\left(\sigma_t^2-\sigma_u^2|\mathcal{F}_u\right)|+|\mathbb{E}\left(\widetilde{\sigma}_t^2-\widetilde{\sigma}_u^2|\mathcal{F}_u\right)|\leq K|t-u|,~~u\leq t,
\end{equation}
\begin{equation}
|\mathbb{E}\left((\sigma_t^2-\sigma_u^2)(\widetilde{\sigma}_t^2-\widetilde{\sigma}_u^2)|\mathcal{F}_u\right)|\leq K|t-u|,~~u\leq t.
\end{equation}
Using these inequalities, we have
\begin{equation}
\left|\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( \int_{\frac{i-1}{n}}^{\frac{i}{n}}\sigma_s^2ds\int_{\frac{i-1}{n}}^{\frac{i}{n}}\widetilde{\sigma}_s^2ds - \frac{1}{n^2}\sigma_{\frac{(j-1)k_n}{n}}^2\widetilde{\sigma}_{\frac{(j-1)k_n}{n}}^2  \right)\right|\leq K\frac{k_n}{n},~~i=(j-1)k_n+1,..,jk_n,
\end{equation}
\begin{equation}
\left|\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( \int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_s^2ds\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\widetilde{\sigma}_s^2ds - \frac{k_n^2}{n^2}\sigma_{\frac{(j-1)k_n}{n}}^2\widetilde{\sigma}_{\frac{(j-1)k_n}{n}}^2  \right)\right|\leq K\frac{k_n}{n}.
\end{equation}
\qedd
\begin{lema}\label{lema_mean_2}
Under assumption SA and $\beta_t=\beta_0$ for $t\in[0,1]$, we have
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|V_j^n(\beta_0) -\frac{n^2}{k_n^2}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_{s}^2ds\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\widetilde{\sigma}_{s}^2ds\right|^2\leq \frac{K}{k_n}.
\end{equation}
\end{lema}
\textbf{Proof of Lemma~\ref{lema_mean_2}.}
We make use of the algebraic identity $x_1y_1-x_2y_2 = (x_1-x_2)(y_1-y_2)+x_2(y_1-y_2)+(x_1-x_2)y_2$, the inequality $\sqrt{xy}\leq\frac{x+y}{2}$ for positive $x,~y$, as well as the boundedness of the processes $\sigma_s^2$ and $\widetilde{\sigma}_s^2$, to bound
\begin{equation}
\begin{split}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|V_j^n(\beta_0) -\frac{n^2}{k_n^2}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_{s}^2ds\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\widetilde{\sigma}_{s}^2ds\right|^2&\leq K\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|V_j^{(n,1)} -\frac{n}{k_n}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_{s}^2ds\right|^2\\&~~+K\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|V_j^{(n,2)}(\beta_0) -\frac{n}{k_n}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\widetilde{\sigma}_{s}^2ds\right|^2.
\end{split}
\end{equation}
Using \Ito lemma, we can write
\begin{equation}
V_j^{(n,1)} -\frac{n}{k_n}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_{s}^2ds = \frac{n}{k_n}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}X_s^ndX_s^c,~~
V_j^{(n,2)} -\frac{n}{k_n}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\widetilde{\sigma}_{s}^2ds = \frac{n}{k_n}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\widetilde{Y}_s^nd\widetilde{Y}_s^c,
\end{equation}
where we used the same notation as in the proof of Lemma~\ref{lema_mean}. From here the result of the lemma follows trivially from an application of Burkholder-Davis-Gundy inequality.
\qedd
\begin{lema}\label{lema_var}
Under assumption SA and $\beta_t=\beta_0$ for $t\in[0,1]$, we have
\begin{equation}
\left|\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( C_j^n(\beta^n)^2 - V_j^n(\beta^n) \right)^2- 2\sigma_{\frac{(j-1)k_n}{n}}^4\widetilde{\sigma}_{\frac{(j-1)k_n}{n}}^4\right|\leq ???.
\end{equation}
\end{lema}
\textbf{Proof of Lemma~\ref{lema_var}.}
We first denote
\begin{equation}
\begin{split}
\overline{C}_j^n &= \frac{n}{\sqrt{k_n}}\sigma_{\frac{(j-1)k_n}{n}}\widetilde{\sigma}_{\frac{(j-1)k_n}{n}}\sum_{i=(j-1)k_n+1}^{jk_n}\Delta_i^nW\Delta_i^n\widetilde{W},\\
\overline{V}_j^n &= \frac{n^2}{k_n^2}\sigma_{\frac{(j-1)k_n}{n}}^2\widetilde{\sigma}_{\frac{(j-1)k_n}{n}}^2\sum_{i=(j-1)k_n+1}^{jk_n}(\Delta_i^nW)^2
\sum_{i=(j-1)k_n+1}^{jk_n}(\Delta_i^n\widetilde{W})^2.
\end{split}
\end{equation}
Using the algebraic identity $x^2-y^2 = (x-y)^2+2y(x-y)$, as well as Cauchy-Schwartz inequality, we can write
\begin{equation}
\begin{split}
&\left|\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( C_j^n(\beta^n)^2 - V_j^n(\beta^n) \right)^2 - \mathbb{E}_{\frac{(j-1)k_n}{n}}\left( (\overline{C}_j^n)^2 - \overline{V}_j^n(\beta^n) \right)^2\right|\\&~~~~~~~~~~~~~~~~~~~~~~~~\leq
K \chi\left(\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( C_j^n(\beta^n)^2 - (\overline{C}_j^n)^2 \right)^2\right) +
K \chi\left(\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( V_j^n(\beta^n) - \overline{V}_j^n \right)^2\right),
\end{split}
\end{equation}
for $\chi(u) = u\vee\sqrt{u}$. We can next bound
\begin{small}
\begin{equation}
\begin{split}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( C_j^n(\beta^n)^2 - (\overline{C}_j^n)^2 \right)^2&\leq 2\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( C_j^n(\beta^n)^2 - C_j^n(\beta_0)^2 \right)^2+2\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( C_j^n(\beta_0)^2 - (\overline{C}_j^n)^2 \right)^2,\nonumber\\
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( V_j^n(\beta^n) - \overline{V}_j^n \right)^2&\leq 2\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( V_j^n(\beta^n) - V_j^n(\beta_0) \right)^2+2\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( V_j^n(\beta_0) - \overline{V}_j^n \right)^2.
\end{split}
\end{equation}
\end{small}
Using the bounds in Lemma~\ref{lema_equic}, we have
\begin{equation}
\left|\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( C_j^n(\beta^n)^2 - C_j^n(\beta_0)^2\right)^2+\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( V_j^n(\beta^n) - V_j^n(\beta_0) \right)^2\right|\leq
Kk_n^2\epsilon_n^2.
\end{equation}
So, we now bound the first terms on the right sides of the inequalities in ???. Using Burkholder-Davis-Gundy inequality for discrete martingales, we have
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|\overline{C}_j^n\right|^p\leq K,~~~\forall p\geq 2.
\end{equation}
Similarly, Burkholder-Davis-Gundy inequality for discrete martingales, together with our assumption for $\sigma_t$ and $\widetilde{\sigma}_t$ being \Ito semimartingales, yield
\begin{small}
\begin{equation}
\begin{split}
&\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|\frac{n}{\sqrt{k_n}}\sum_{i=(j-1)k_n+1}^{jk_n}\left[\left(\Delta_i^nX^c-\sigma_{\frac{(j-1)k_n}{n}}\Delta_i^nW\right)
\Delta_i^n\widetilde{Y}^c + \sigma_{\frac{(j-1)k_n}{n}}\Delta_i^nW\left(\Delta_i^n\widetilde{Y}^c-\widetilde{\sigma}_{\frac{(j-1)k_n}{n}}\Delta_i^n\widetilde{W}\right)
\right]\right|^p\\&~~~~~~~~~~~~~\leq K\left(\frac{k_n}{n}\right)^{p/2}.
\end{split}
\end{equation}
\end{small}
Combining the above two inequalities, together with Cauchy-Schwartz inequality, we get
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( C_j^n(\beta_0)^2 - (\overline{C}_j^n)^2 \right)^2\leq K\frac{k_n}{n},
\end{equation}
and this bound can be further improved but suffices for our purposes here.

We turn next to bounding $\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( V_j^n(\beta_0) - \overline{V}_j^n \right)^2$. Using inequality in means, we first have
\begin{small}
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left(\frac{n}{k_n}\sum_{i=(j-1)k_n+1}^{jk_n}\left[(\Delta_i^nX^c)^2+(\Delta_i^n\widetilde{Y}^c)^2
+\sigma_{\frac{(j-1)k_n}{n}}^2(\Delta_i^nW)^2 + \widetilde{\sigma}_{\frac{(j-1)k_n}{n}}^2(\Delta_i^n\widetilde{W})^2\right]  \right)^p\leq K.
\end{equation}
\end{small}
Using the algebraic identity $x^2-y^2 = (x-y)^2+2y(x-y)$, the Burkholder-Davis-Gundy inequality for discrete martingales, \Ito formula for the function $f(x,y) = x y$, our assumption for $\sigma_t$ being \Ito semimartingale, we have
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|\frac{n}{k_n}\sum_{i=(j-1)k_n+1}^{jk_n}\left[(\Delta_i^nX^c)^2-\sigma_{\frac{(j-1)k_n}{n}}^2(\Delta_i^nW)^2\right]\right|^p\leq K\frac{k_n}{n},~~~\forall p\geq 2,
\end{equation}
and we have similarly
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|\frac{n}{k_n}\sum_{i=(j-1)k_n+1}^{jk_n}\left[(\Delta_i^n\widetilde{Y}^c)^2
-\widetilde{\sigma}_{\frac{(j-1)k_n}{n}}^2(\Delta_i^n\widetilde{W})^2\right]\right|^p\leq K\frac{k_n}{n},~~~\forall p\geq 2.
\end{equation}
Using the above inequalities and \Holder~ inequality, we have
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( V_j^n(\beta_0) - \overline{V}_j^n \right)^2\leq K\left(\frac{k_n}{n}\right)^{1-\iota},~~~~\forall \iota>0.
\end{equation}
Altogether, combining the bounds in ???, ??? and ???, we get
\begin{equation}
\begin{split}
\left|\mathbb{E}_{\frac{(j-1)k_n}{n}}\left( C_j^n(\beta^n)^2 - V_j^n(\beta^n) \right)^2 - \mathbb{E}_{\frac{(j-1)k_n}{n}}\left( (\overline{C}_j^n)^2 - \overline{V}_j^n(\beta^n) \right)^2\right|\leq
K \left(k_n\epsilon_n\bigwedge \left(\frac{k_n}{n}\right)^{1-\iota}\right).
\end{split}
\end{equation}
We are thus left with $\mathbb{E}_{\frac{(j-1)k_n}{n}}\left((\overline{C}_j^n)^2-\overline{V}_j^n\right)^2$. First, we have
\begin{equation}
\frac{\frac{(\overline{C}_j^n)^2}{\overline{V}_j^n}}{1-\frac{1}{k_n}\frac{(\overline{C}_j^n)^2}{\overline{V}_j^n}} ~\stackrel{d}{=}~t_{k_n}^2~~~\Longrightarrow
\frac{(\overline{C}_j^n)^2}{\overline{V}_j^n}~\stackrel{d}{=}~\frac{t_{k_n}^2}{1+\frac{1}{k_n}t_{k_n}^2}.
\end{equation}
Therefore, for $k_n>4$, using the properties of the t distribution, we have
\begin{equation}
\left|\mathbb{E}_{\frac{(j-1)k_n}{n}}\left(\frac{(\overline{C}_j^n)^2}{\overline{V}_j^n}-2\right)^2-1\right|\leq \frac{K}{k_n}.
\end{equation}
Second, using Burkholder-Davis-Gundy inequality for discrete martingales, we have
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left(\left( \overline{V}_j^n \right)^2 - \sigma_{\frac{(j-1)k_n}{n}}^4\widetilde{\sigma}_{\frac{(j-1)k_n}{n}}^4\right)^p\leq \frac{K}{k_n^{p/2}},~~~\forall p\geq 2.
\end{equation}
Combining the above bounds, we have
\begin{equation}
\left| \mathbb{E}_{\frac{(j-1)k_n}{n}}\left((\overline{C}_j^n)^2-\overline{V}_j^n\right)^2 - 2 \sigma_{\frac{(j-1)k_n}{n}}^4\widetilde{\sigma}_{\frac{(j-1)k_n}{n}}^4 \right|\leq \frac{K}{\sqrt{k_n}}.
\end{equation}
\qedd
\begin{lema}\label{lema_powers}
Under assumption SA and $\beta_t=\beta_0$ for $t\in[0,1]$, for any fixed $\alpha>0$, we have
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|C_j^n(\beta^n)\right|^p\leq K(1\vee k_n^{p/2}\epsilon^p),~~\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|V_j^n(\beta^n)\right|^p\leq K,
\end{equation}
\begin{equation}
\mathbb{P}\left(\left| V_{j}^{(n,1)} - \frac{n}{k_n}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_{s}^2ds \right|\geq \alpha \frac{n}{k_n} \int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_{s}^2ds\right)\leq \frac{K}{k_n^{p/2}},~~\forall p\geq 1,
\end{equation}
\begin{equation}
\mathbb{P}\left(\left| V_{j}^{(n,2)}(\beta_0) - \frac{n}{k_n}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\widetilde{\sigma}_{s}^2ds \right|\geq \alpha \frac{n}{k_n} \int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\widetilde{\sigma}_{s}^2ds\right)\leq \frac{K}{k_n^{p/2}},~~\forall p\geq 1.
\end{equation}
\end{lema}
\textbf{Proof of Lemma~\ref{lema_powers}.}
\begin{equation}
\begin{split}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|C_j^n(\beta^n)\right|^p&\leq K\epsilon_n^p\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|\frac{n}{\sqrt{k_n}}\sum_{i=(j-1)k_n+1}^{jk_n}(\Delta_i^nX^c)^2\right|^p\\&~~+K\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|
\frac{n}{\sqrt{k_n}}\sum_{i=(j-1)k_n+1}^{jk_n}(\Delta_i^nX^c\Delta_i^n\widetilde{Y}^c)\right|^p.
\end{split}
\end{equation}
Inequality in means implies
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|\frac{n}{\sqrt{k_n}}\sum_{i=(j-1)k_n+1}^{jk_n}(\Delta_i^nX^c)^2\right|^p\leq Kk_n^{p/2},
\end{equation}
and Burkholder-Davis-Gundy inequality for discrete martingales gives
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|
\frac{n}{\sqrt{k_n}}\sum_{i=(j-1)k_n+1}^{jk_n}(\Delta_i^nX^c\Delta_i^n\widetilde{Y}^c)\right|^p\leq K.
\end{equation}
Combining these results, we get the first part of ???. The second result in ??? follows from Cauchy-Schwartz inequality together with inequality in means.

We next show ??? with ??? shown in exactly the same way. Using the notation in the proof of Lemma~\ref{lema_mean}, we have
\begin{equation}
V_j^{(n,1)}-\frac{n}{k_n}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_{s}^2ds = 2\frac{n}{k_n}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}X_{s}^ndX_s,
\end{equation}
and therefore by an application of Burkholder-Davis-Gundy inequality
\begin{equation}
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|V_j^{(n,1)}-\frac{n}{k_n}\int_{\frac{(j-1)k_n}{n}}^{\frac{jk_n}{n}}\sigma_{s}^2ds\right|^p\leq \frac{K}{k_n^{p/2}},~~\forall p\geq 1.
\end{equation}
\qedd

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{lema}\label{lema_equic}
Under assumption SA and $\beta_t=\beta_0$ for $t\in[0,1]$, for any $x$ and $y$ bounded by a constant and $p>1$, we have
\begin{equation}
\left\{\begin{array}{l}
\left|\mathbb{E}_{\frac{(j-1)k_n}{n}}\left(C_j^n(x\beta^n)^2 - C_j^n(y\beta^n)^2 \right)\right|\leq K|x-y|\left(\epsilon_n^2k_n+\epsilon_n\frac{k_n}{\sqrt{n}}\right),\\
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|C_j^n(x\beta^n)^2 - C_j^n(y\beta^n)^2 \right|^p\leq K|x-y|^{p}k_n^p(\epsilon_n^p\vee\epsilon_n^{2p}),\\
\mathbb{E}_{\frac{(j-1)k_n}{n}}\left|V_j^n(x\beta^n) - V_j^n(y\beta^n) \right|^p\leq K|x-y|^{p}(\epsilon_n^p\vee\epsilon_n^{2p}),
\end{array}\right.
\end{equation}
and
\begin{equation}
\left\{\begin{array}{l}
\mathbb{E}\left|\sqrt{\frac{k_n}{n}}\sum_{j=1}^{\lfloor n/k_n\rfloor}\left(C_j^n(x\beta^n)^2-C_j^n(y\beta^n)^2\right)\right|^p\leq K|x-y|^pk_n^p(\epsilon_n^p\vee\epsilon_n^{2p}),\\
\mathbb{E}\left|\sqrt{\frac{k_n}{n}}\sum_{j=1}^{\lfloor n/k_n\rfloor}\left(V_j^n(x\beta^n)-V_j^n(y\beta^n)\right)\right|^p\leq K|x-y|^p\left(\frac{n}{k_n}\right)^{p/2}(\epsilon_n^p\vee\epsilon_n^{2p}).
\end{array}\right.
\end{equation}
\end{lema}
\textbf{Proof of Lemma~\ref{lema_equic}.}
We can split
\begin{equation}
\begin{split}
&\frac{k_n}{n^2}\left(C_j^n(x\beta^n)^2 - C_j^n(y\beta^n)^2\right) \\&~~~~~= (x^2-y^2)\epsilon_n^2\sum_{i,k:~i\neq k}(\Delta_i^nX^c)^2(\Delta_k^nX^c)^2+(x-y)\epsilon_n\sum_{i,k:~i<k}\Delta_i^nX^c\Delta_i^n\widetilde{Y}^c(\Delta_k^nX^c)^2\\&~~~~~~~~+
(x-y)\epsilon_n\sum_{i,k:~i<k}(\Delta_i^nX^c)^2\Delta_k^nX^c\Delta_k^n\widetilde{Y}^c+(x^2-y^2)\epsilon_n^2\sum_i(\Delta_i^nX^c)^4\\&~~~~~~~~
+2(x-y)\epsilon_n\sum_{i}(\Delta_i^nX^c)^3\Delta_i^n\widetilde{Y}^c,
\end{split}
\end{equation}
where in the above summation $i=(j-1)k_n+1,...,jk_n$ and $k=(j-1)k_n+1,...,jk_n$. From here, using the inequalities ???-??? in the proof of Lemma~
\ref{lema_mean}, we have the first bound in ???. Upon using inequality in means, we have the second part of ???.

Turning to the last part of ???, we can split
\begin{small}
\begin{equation}
\begin{split}
&\frac{k_n^2}{n^2}\left(V_j^n(x\beta^n) - V_j^n(y\beta^n)\right) \\&~~~~~= \left(\sum_{i=(j-1)k_n+1}^{jk_n}(\Delta_i^nX^c)^2\right)\left(\sum_{i=(j-1)k_n+1}^{jk_n}\left\{(x^2-y^2)\epsilon_n^2(\Delta_i^nX^c)^2+2(x-y)\epsilon_n
\Delta_i^n\widetilde{Y}^c\Delta_i^nX^c\right\}
\right).
\end{split}
\end{equation}
\end{small}
Using equality in means we have,
\[\mathbb{E}_{\frac{(j-1)k_n}{n}}\left(\frac{n}{k_n}\sum_{i=(j-1)k_n+1}^{jk_n}(\Delta_i^nX^c)^2\right)^q\leq K,~~~\forall q>1.\]
From here, using \Holder~ inequality and inequality in means, we have the last part of ???.

We now establish ???. We use the inequality
\begin{equation}
\begin{split}
&\left|\sqrt{\frac{k_n}{n}}\sum_{j=1}^{\lfloor n/k_n\rfloor}(C_j^n(x\beta^n)^2-C_j^n(y\beta^n)^2)\right|^p\\&~~~~~~~~~~~~~~\leq K\left|\sqrt{\frac{k_n}{n}}\sum_{j=1}^{\lfloor n/k_n\rfloor}\left[(C_j^n(x\beta^n)^2-C_j^n(y\beta^n)^2) - \mathbb{E}_{\frac{(j-1)k_n}{n}}(C_j^n(x\beta^n)^2-C_j^n(y\beta^n)^2) \right]\right|^p\\&~~~~~~~~~~~~~~~~+K\left|\sqrt{\frac{k_n}{n}}\sum_{j=1}^{\lfloor n/k_n\rfloor}\mathbb{E}_{\frac{(j-1)k_n}{n}}(C_j^n(x\beta^n)^2-C_j^n(y\beta^n)^2)\right|^p.
\end{split}
\end{equation}
From here, for the first term on the right side of the above inequality, we can use Burkholder-Davis-Gundy inequality for discrete martingales, together with the second bound in ???. For the second term on the right side of the above inequality we can use the first bound in ??? as well as inequality in means. Combining these results, we get the bound in ???.

The last part of ??? follows from inequality in means and the last bound in ???.
\qedd

%\begin{equation}
%\sup_{\beta:|\beta-\beta_0|\leq \beta_0n^{-1/2+\iota}}|T^{(n,1)}(\beta)-T^{(n,1)}(\beta_0)|~\stackrel{\mathbb{P}}{\longrightarrow}~0
%\end{equation}

